SafeAug: Safety-Critical Driving Data Augmentation from Naturalistic Datasets

Safety-critical driving data is crucial for developing safe and trustworthy self-driving algorithms. Due to the scarcity of safety-critical data in naturalistic datasets, current approaches primarily utilize simulated or artificially generated images. However, there remains a gap in authenticity between these generated images and naturalistic ones. We propose a novel framework to augment the safety-critical driving data from the naturalistic dataset to address this issue. In this framework, we first detect vehicles using YOLOv5, followed by depth estimation and 3D transformation to simulate vehicle proximity and critical driving scenarios better. This allows for targeted modification of vehicle dynamics data to reflect potentially hazardous situations. Compared to the simulated or artificially generated data, our augmentation methods can generate safety-critical driving data with minimal compromise on image authenticity. Experiments using KITTI datasets demonstrate that a downstream self-driving algorithm trained on this augmented dataset performs superiorly compared to the baselines, which include SMOGN and importance sampling.

==> u.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{acceleration.jpg}
    \caption{Distribution of Acceleration}
    \label{fig:acceleration}
\end{figure}

\begin{figure*}[ht]
\centering
\begin{minipage}{.24\textwidth}
\centering
\includegraphics[width=\linewidth]{allimage.png}
\caption*{Original}
\end{minipage}
\hfill
\begin{minipage}{.24\textwidth}
\centering
\includegraphics[width=\linewidth]{smote.png}
\caption*{SMOTE}
\end{minipage}
\hfill
\begin{minipage}{.24\textwidth}
\centering
\includegraphics[width=\linewidth]{imporsam.png}
\caption*{Importance sampling}
\end{minipage}
\hfill
\begin{minipage}{.24\textwidth}
\centering
\includegraphics[width=\linewidth]{ours.png}
\caption*{Ours}
\end{minipage}
\caption{Distribution of Acceleration}
\label{fig:sunny_day_frames}
\end{figure*}



\begin{figure*}[ht]
\centering
\begin{minipage}{.45\textwidth}
\centering
\includegraphics[width=\linewidth]{allimage.png}
\caption*{Original}
\end{minipage}
\hfill
\begin{minipage}{.45\textwidth}
\centering
\includegraphics[width=\linewidth]{ours.png}
\caption*{Ours}
\end{minipage}

\vspace{3mm} 

\begin{minipage}{.45\textwidth}
\centering
\includegraphics[width=\linewidth]{smote.png}
\caption*{SMOTE}
\end{minipage}
\hfill
\begin{minipage}{.45\textwidth}
\centering
\includegraphics[width=\linewidth]{imporsam.png}
\caption*{Importance sampling}
\end{minipage}
\caption{Distribution of Acceleration}
\label{fig:sunny_day_frames}
\end{figure*}


\subsection{Augmentation for unbalance datasets}
upsampling \tcr{starting with the classic data augmentation in image classification tasks, such as rotation. Then introduce data augmentation in driving data, such as importance sampling and SMOTE.}

In order to mitigate the problems posed by unbalanced datasets, several strategies have been devised, focusing mainly on enhancing the representation of a few categories during the training process of machine learning models. Data-level techniques are widely used, including resampling or data augmentation. Resampling can either increase its instances by oversampling minorities or reduce its instances by undersampling majorities. Synthetic Minority Oversampling Technique (SMOTE)\cite{Chawla_2002} is a notable method in oversampling that creates synthetic samples rather than just replicating existing samples. On the other hand, data enhancement techniques generate new data points through transformations such as rotations and flips, which help to enhance minority categories and provide more diverse examples for model training.

Algorithmic-level techniques are another important category that adjust the learning process to counteract bias against most categories. Examples include importance sampling\cite{kloek1978bayesian}, Cost-sensitive learning\cite{Ling2010}, and ensemble methods (e.g., boosting and bagging). These methods typically involve creating multiple subsets of data and ensuring that each subset provides a balanced view so that the combined model has better generalization across different class distributions. These techniques typically yield good results in creating robust models that are sensitive to all categories, especially in critical applications such as autonomous driving.

\subsection{Augmentation for driving datasets}

In recent years, specialized techniques for data augmentation and simulation have become critical for training autonomous driving systems to handle safety-critical scenarios. Several innovative approaches are reviewed here that aim to generate synthetic driving scenarios, enhance dataset diversity, and simulate corner cases to improve the ability of models to predict and respond to real-world driving challenges.

Technologies such as AdvSim \cite{wang2023advsim}, KING\cite{hanselmann2022king}, and Adv3D\cite{sarva2023adv3d} focus on generating synthetic data that simulates safety-critical scenarios, often involving potential collisions or dangerous driving conditions. These approaches use simulation to enhance the realism and applicability of scenarios to realistic conditions. For example, AdvSim \cite{wang2023advsim} updates LiDAR sensor data in a simulated environment to create hazardous driving scenarios, which are critical for testing and improving vehicle response under duress. Similarly, KING \cite{hanselmann2022king} utilizes kinematic gradients in the simulation environment to generate scenarios specifically geared towards collision avoidance, thereby enhancing the model's predictive capabilities in high-risk situations. Some Techniques\cite{WANG2020257} \cite{alhaija2017augmented} focus on augmenting real-world images or generating entirely new images containing challenging driving conditions. These methods change the background scene, lighting and weather conditions, and introduce occlusions to create diverse and challenging datasets.

SIMBAR \cite{Zhang_2022_CVPR} and SurfelGAN \cite{Yang_2020_CVPR} are examples of methods that manipulate sensor inputs and environmental conditions (e.g., lighting) to simulate different times of the day or weather conditions to create richer, more diverse training data. These methods aim to prepare driving models for the variability and unpredictability of real-world driving. Some studies, such as RADAR\cite{9896871} and TauAud\cite{9742083}, focus on augmenting the data by altering the driving style or testing the robustness of the image recognition system in adverse weather conditions. These approaches enrich the scenarios of the dataset, test the limits of current autonomous driving systems and ensure that the system can effectively handle unexpected situations.


\section{Problem Statement}

The objective of this research is to enhance the realism and applicability of datasets for autonomous driving system training. Traditional datasets often lack sufficient representation of hazardous scenarios essential for developing robust predictive models. Our approach involves augmenting images from the KITTI dataset, denoted by \( I \), to include scenarios that simulate more dangerous conditions, thereby producing \( I_{\text{aug}} \). 
\begin{equation*}
I_{\text{aug}}(i) \leftarrow I(i)
\end{equation*}

The augmentation process begins with each raw image \( I(i) \) undergoing depth estimation and vehicle detection to create depth and tagged images respectively. These are then used to generate a 3D model of the scene, which is manipulated to simulate hazardous driving conditions by adjusting vehicle distances. This modified 3D model is then converted back into a 2D augmented image, \( I_{\text{aug}}(i) \).

For testing, we compare the performance of a model trained under different scenarios:
1. Using the original images, \( I \).
2. Using the original images, \( I \), augmented by other methods, as baselines.
3. Using a combination of original and augmented images, \( I + I_{\text{aug}} \).

The model’s accuracy in predicting vehicle acceleration is assessed, particularly focusing on handling safety-critical driving data, which represent the most challenging driving scenarios. The comparison aims to determine if the inclusion of \( I_{\text{aug}} \) enhances the model’s ability to predict critical outcomes in real-world hazardous conditions more effectively than baseline methods. We define the training optimization for our downstream car-following model as:
\begin{equation*}
\theta^* = \arg\min_{\theta} D(\theta; I + I_{\text{aug}})
\end{equation*}
Here, \( \theta^* \) denotes the optimal model parameters, and \( D(\theta; I + I_{\text{aug}}) \) quantifies the deviation of model predictions from the true vehicle accelerations under both baseline and augmented conditions.

